3D Head-Position Prediction in First-Person View by Considering Head Pose for Human-Robot Eye Contact

For a humanoid robot to make eye contact and initiate communication with a person, it is necessary to estimate the person's head position. However, eye contact becomes difficult due to the mechanical delay of the robot when the person is moving. Owing to these issues, it is important to conduct a head-position prediction to mitigate the effect of the delay in the robot motion. Based on the fact that humans turn their heads before changing direction while walking, we hypothesized that the accuracy of three-dimensional (3D) head-position prediction from a first-person view can be improved by considering the head pose. We compared our method with a conventional Kalman filter-based approach, and found our method to be more accurate. The experiment results show that considering the head pose helps improve the accuracy of 3D head-position prediction.

==> experiments.tex <==
\section{Experiments}
In this section, we compare the proposed method with the baseline method, the Kalman filter, using data taken of a subject who is assumed to be a passerby walking.
The experiment in which the subject's walking is photographed is called the data acquisition experiment, and the experiment in which the methods are compared using the data is called the validation experiment.

\subsection{Data Acquisition Experiment}
In this section, we describe the details of the data acquisition experiment.
The purpose of this experiment was to obtain a data set of RGB-D videos of the subject while walking.
The experimental environment is as shown in Fig~\ref{fig:env}
.
\begin{figure}[hbtp]
    \includegraphics[width=\linewidth]{figures/env}
    \caption{The overhead view of the experimental environment.}
    \label{fig:env}
\end{figure}
\begin{figure}[hbtp]
    \includegraphics[width=\linewidth]{figures/front}
    \caption{Photograph taken from the azure kinect in the actual environment.}
    \label{fig:front}
\end{figure}
In the room, we set up three landmark desks and an azure kinect.
The rooms are separated by partitions, so that each landmark is not directly visible from the other landmarks.
The size of the room is 7.3m x 9.0m square as shown in Fig~\ref{fig:env}
.
Data acquisition experiments were conducted with a total of 13 subjects.
The route of R1-6 for the subjects to walk is shown in Fig~\ref{fig:env}
, and there are desks for landmarks at the beginning and end of the route.
In this experiment, the depth mode of Azure Kinect was set to NFOV 2x2 Binned (SW).
For NFOV 2x2 Binned (SW), the operating range is from 0.5 to 5.46 m.
The videos were taken at 30 fps.
The procedure of the experiment is as follows.
\begin{itemize}
    \item The subjects were instructed to walk naturally along the route R1 as shown in the figure.
    \item The experimenter instructed when to start walking the route, and at the same time, the azure kinect started taking pictures.
    \item When the subject reached the destination of the route, the experimenter ended the shooting and instructed the subject to finish walking.
    \item The above procedure was repeated for R2-6 as well.
\end{itemize}
In this experiment, we obtained a total of 78 videos, each about 5 seconds long.
\subsection{Validation Experiment}
In this section, we describe the contents of the validation experiment.
The purpose of the evaluation experiment is to compare the accuracy of our method and the conventional Kalman filter prediction (hereafter referred to as the baseline method) on the acquired video data set.
We used the data within the operating range of these.
The horizontal angle of the waist was defined as moving direction, and the difference between the horizontal angle of the waist and the horizontal angle of the face was defined as the angle of face orientation.
The procedure of the experiment is as follows.
\begin{itemize}
    \item From the acquired video dataset, we used the azure kinect body-tracking SDK to extract the positions of the face and waist and their quaternions, and to detect the face direction and movement direction for each frame.
    \item These two values were input to the proposed method and the baseline method, and the predicted values after 0.5s, or 15steps in our setting, were calculated for each frame.
\end{itemize}
The values obtained by the azure kinect body-tracking SDK will be referred to as observed values.
For the routes R1-6 set in the data acquisition experiment, we group the left and right target routes. We call the group of R1 and R2 as R12, R3 and R4 as R34, and R5 and R6 as R56.
Map the calculated positions to the symbols as follows.
\begin{itemize}
    \item[(a)] Estimated position with Kalman filter applied to the observed position of the face.
    \item[(b)] Predicted location of face by baseline method
    \item[(c)] Predicted location of the face by the proposed method
\end{itemize}
The validation method is described below.
\begin{itemize}
    \item The error between (b) and (a), and the error between (c) and (a) were calculated for the entire movie, and the total error and the number of frames of the movie were obtained. 
    \item For each group, we obtained the average of the errors for all videos. 
    \item For each group, the means were compared between the baseline and the proposed method, and one-tailed tests of wilcoxon signed rank tests were performed.
\end{itemize}
The error was calculated using the Euclidean distance.

The hypotheses to be tested in this experiment are as follows.
\begin{itemize}
    \item For the turning route (R3-6), "the accuracy of the proposed method is better than that of the baseline method because the face direction is considered to precede the direction of travel and look toward the destination when turning".
    \item For the straight route (R1-2), "the results of the baseline method and the proposed method are almost identical because the face direction is always considered to match the direction of travel".
\end{itemize}
